Robust and Efficient 3D Gaussian Splatting for Urban Scene Reconstruction

We present a framework that enables fast reconstruction and real-time rendering of urban-scale scenes while maintaining robustness against appearance variations across multi-view captures. Our approach begins with scene partitioning for parallel training, employing a visibility-based image selection strategy to optimize training efficiency. A controllable level-of-detail (LOD) strategy explicitly regulates Gaussian density under a user-defined budget, enabling efficient training and rendering while maintaining high visual fidelity. The appearance transformation module mitigates the negative effects of appearance inconsistencies across images while enabling flexible adjustments. Additionally, we utilize enhancement modules, such as depth regularization, scale regularization, and antialiasing, to improve reconstruction fidelity. Experimental results demonstrate that our method effectively reconstructs urban-scale scenes and outperforms previous approaches in both efficiency and quality. The source code is available at: https://yzslab.github.io/REUrbanGS.

==> sec/3_preliminaries.tex <==
\section{Preliminaries}


3DGS \cite{kerbl20233d} represents a scene using a set of explicit 3D Gaussians. Each 3D Gaussian is defined by: 
\begin{equation}
    G(x)=e^{-\frac{1}{2}(x-\mu)^{T}\Sigma^{-1}(x-\mu)}
\end{equation}
where $\mu$ is the center and $\Sigma$ is the covariance matrix. 

To render an image, the 3D Gaussians are first projected onto the image plane, forming 2D Gaussians $G^{'}(x)$. These are then processed in sequence, based on their depth ordering, to compute the color of each pixel using $\alpha$-blending.

During the training process, 3DGS periodically performs a densification operation on those Gaussians that exhibit relatively high mean gradients in the image space, thereby improving their ability to capture the underlying geometry. As described in \cite{kerbl20233d}, the loss function of 3DGS includes the L1 and D-SSIM metrics, computed between the rendered image $\predimage$ and its corresponding ground-truth image $\gtimage$:
\begin{equation}
    \label{eq:3dgs-loss}
    \mathcal{L} = (1-\lambda_{\textrm{}})\mathcal{L}_{1}(\gtimage, \predimage) + \lambda_{\textrm{}}\mathcal{L}_{\textrm{D-SSIM}}(\gtimage, \predimage)
\end{equation}
where $\lambda_{\textrm{}}$ is a hyperparameter, which is set to 0.2 in \cite{kerbl20233d}.


By optimizing the attributes of the Gaussians and carrying out densification to minimize this loss, 3DGS ultimately fulfills its goal of reconstructing the target scene.

